DOCTOR: A Simple Method for Detecting Misclassification Errors

Deep neural networks (DNNs) have shown to perform very well on large scale object recognition problems and lead to widespread use for real-world applications, including situations where DNN are implemented as "black boxes". A promising approach to secure their use is to accept decisions that are likely to be correct while discarding the others. In this work, we propose DOCTOR, a simple method that aims to identify whether the prediction of a DNN classifier should (or should not) be trusted so that, consequently, it would be possible to accept it or to reject it. Two scenarios are investigated: Totally Black Box (TBB) where only the soft-predictions are available and Partially Black Box (PBB) where gradient-propagation to perform input pre-processing is allowed. Empirically, we show that DOCTOR outperforms all state-of-the-art methods on various well-known images and sentiment analysis datasets. In particular, we observe a reduction of up to $4\%$ of the false rejection rate (FRR) in the PBB scenario. DOCTOR can be applied to any pre-trained model, it does not require prior information about the underlying dataset and is as simple as the simplest available methods in the literature.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please, refer to~\cref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We briefly discuss societal impacts or our work in~\cref{sec:conclusion}. Furthermore, to the best of our knowledge, the current application of our framework and the utilized data do not raise any ethical concerns. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{The full body of theoretical statements and results is reported in~\cref{sec:performanceandmetrics}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{The full body of proofs for the theoretical results is reported in~\cref{appendix:proofs}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{A link to the code repository is provided in page 6. Instructions to run the aforementioned code and reproduce the results is provided within the repository as a README.md file.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{Models' training phase not needed in the proposed framework.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{Only for experiments including randomness in the data we repeated several runs on different instances and expressed the results in terms of mean and standard deviation. In addition, in the code repository (cf. 3.a) we provide the datasets we used for the experiments or a link to them.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Cf.~\cref{appendix:enviroment}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We only used openly available code which we carefully referred throughout the paper.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{A link to the code repository and related instructions is provided in page 6.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We utilized standard benchmark openly available datasets.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> figures/fig_all_cifar100.tex <==
\begin{figure*}[!htb]
	\centering
	\begin{subfigure}[b]{  0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{   $T=1$}
	    \label{fig:cifar100_T_1_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1.1_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=1.1$}
% 	    \label{fig:cifar100_T_1.1_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1.2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=1.2$}
% 	    \label{fig:cifar100_T_1.2_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{  0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1.3_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{   $T=1.3$}
	    \label{fig:cifar100_T_1.3_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1.4_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=1.4$}
% 	    \label{fig:cifar100_T_1.4_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{  0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1.5_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{   $T=1.5$}
	    \label{fig:cifar100_T_1.5_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=2$}
% 	    \label{fig:cifar100_T_2_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall2.5_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=2.5$}
% 	    \label{fig:cifar100_T_2.5_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall3_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=3$}
% 	    \label{fig:cifar100_T_3_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{  0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall100_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{   $T=100$}
% 	    \label{fig:cifar100_T_100_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{  0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/cifar100_overall1000_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{   $T=1000$}
	    \label{fig:cifar100_T_1000_all}
	\end{subfigure}
	\caption{CIFAR100}
	\label{fig:auc_cifar100_all}
\end{figure*}

==> figures/fig_all_svhn.tex <==
\begin{figure*}[!htb]
	\centering
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1$}
	    \label{fig:svhn_T_1_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1.1_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.1$}
% 	    \label{fig:svhn_T_1.1_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1.2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.2$}
% 	    \label{fig:svhn_T_1.2_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1.3_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1.3$}
	    \label{fig:svhn_T_1.3_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1.4_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.4$}
% 	    \label{fig:svhn_T_1.4_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1.5_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1.5$}
	    \label{fig:svhn_T_1.5_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=2$}
% 	    \label{fig:svhn_T_2_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall2.5_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=2.5$}
% 	    \label{fig:svhn_T_2.5_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall3_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=3$}
% 	    \label{fig:svhn_T_3_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall100_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=100$}
% 	    \label{fig:svhn_T_100_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/svhn_overall1000_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1000$}
	    \label{fig:svhn_T_1000_all}
	\end{subfigure}
	\caption{SVHN}
	\label{fig:auc_svhn_all}
\end{figure*}

==> figures/fig_all_tiny.tex <==
\begin{figure*}[!htb]
	\centering
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1$}
	    \label{fig:tinyimagenet_T_1_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1.1_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.1$}
% 	    \label{fig:tinyimagenet_T_1.1_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1.2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.2$}
% 	    \label{fig:tinyimagenet_T_1.2_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1.3_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1.3$}
	    \label{fig:tinyimagenet_T_1.3_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1.4_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=1.4$}
% 	    \label{fig:tinyimagenet_T_1.4_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1.5_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1.5$}
	    \label{fig:tinyimagenet_T_1.5_all}
	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall2_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=2$}
% 	    \label{fig:tinyimagenet_T_2_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall2.5_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=2.5$}
% 	    \label{fig:tinyimagenet_T_2.5_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall3_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=3$}
% 	    \label{fig:tinyimagenet_T_3_all}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{ 0.23\textwidth}
% 	    \centering
% 	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall100_pt__.png}
% 	    \vspace{-1.5\baselineskip}
% 	    \caption{ $T=100$}
% 	    \label{fig:tinyimagenet_T_100_all}
% 	\end{subfigure}
	\begin{subfigure}[b]{ 0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/plots_appendix/tinyimagenet_overall1000_pt__.png}
	    \vspace{-1.5\baselineskip}
	    \caption{ $T=1000$}
	    \label{fig:tinyimagenet_T_1000_all}
	\end{subfigure}
	\caption{TinyImageNet}
	\label{fig:auc_tinyimagenet_all}
\end{figure*}

==> figures/fig_best_risk.tex <==
\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.3]{figures/plots/rc_cifar10.pdf}
	    \caption{}
	    \label{fig:cifar10_risk}
	\end{subfigure}
	\begin{subfigure}[b]{0.3\textwidth}
	\centering
	    \includegraphics[scale=0.3]{figures/plots/rc_cifar100.pdf}
		\caption{}
	    \label{fig:cifar100_risk}
	\end{subfigure}
	%\includegraphics[scale=0.3]{figures/plots/tinyimagenetbest.pdf}\\
	%(a) \hspace{4.5cm}(b) \hspace{4.5cm}(c)\\
	%\includegraphics[scale=0.3]{figures/plots/fashionbest.pdf}
	%\includegraphics[scale=0.3]{figures/plots/softwarebest.pdf}\\
	%(d) \hspace{4.5cm}(e)
	\caption{Comparison between the best result of our method (in green) and Softmax Response (in red) on CIFAR10,  CIFAR100, TinyImageNet, Amazon Fashion and Amazon Software w.r.t. risk-coverage curve. As can be seen, our methodology outperforms Softmax Response.}
	\label{fig:best_risk}
\end{figure*}

==> figures/fig_perturbations.tex <==
\begin{figure}[!htb]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/cifar10_best_eps_1_2.png}
	    \vspace{-1.5\baselineskip}
	    \caption{CIFAR10}
	    \label{fig:eps_cifar10}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/cifar100_best_eps_1_2.png}
	    \vspace{-1.5\baselineskip}
	    \caption{CIFAR100}
	    \label{fig:eps_cifar100}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/tinyimagenet_best_eps_1_2.png}
	    \vspace{-1.5\baselineskip}
	    \caption{TinyImageNet}
	    \label{fig:eps_tiny}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/svhn_best_eps_1_2.png}
	    \vspace{-1.5\baselineskip}
	    \caption{SVHN}
	    \label{fig:eps_svhn}
	\end{subfigure}
	\caption{AUROCs on CIFAR10, CIFAR100, TinyImageNet and SVHN when $T=1000$ and $0\leq\epsilon\leq0.004$. The red point marks the best value of the AUROC obtained through $D_\alpha$ under TBB.}
	\label{fig:epsilons_auroc}
\end{figure}



==> figures/fig_perturbations_doctor.tex <==
\begin{figure}[!htb]
	\centering
	\begin{subfigure}[b]{0.23\textwidth}
	    \centering
x	    \includegraphics[width=\textwidth]{figures/plots/cifar10_eps_auroc.png}
	    \vspace{-1.5\baselineskip}
	    \caption{CIFAR10: $T=1$}
	    \label{fig:cifar10_best_eps}
	\end{subfigure}
	\begin{subfigure}[b]{0.23\textwidth}
	    \centering
x	    \includegraphics[width=\textwidth]{figures/plots/cifar100_eps_auroc.png}
	    \vspace{-1.5\baselineskip}
	    \caption{CIFAR100: $T=1$}
	    \label{fig:cifar100_best_eps}
	\end{subfigure}
	\begin{subfigure}[b]{0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/tinyimagenet_best_eps.png}
	    \vspace{-1.5\baselineskip}
	    \caption{TinyImageNet: $T=1$}
	    \label{fig:tiny_best_eps}
	\end{subfigure}
	\begin{subfigure}[b]{0.23\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{figures/plots/svhn_best_eps.png}
	    \vspace{-1.5\baselineskip}
	    \caption{SVHN: $T=1$}
	    \label{fig:svhn_best_eps}
	\end{subfigure}
	\caption{AUROCs obtained via $D_\alpha$ according to the best value of $T$ and by varying $\epsilon$ as in~\cref{tab:best_eps_alpha}.}
	\label{fig:auc}
\end{figure}

==> rebuttal/table_miss.tex <==
\begin{table}[!htb]
\centering
	\caption{For all methods, in TBB, we set $T=1$ and $\epsilon=0$; in PBB we set : $\epsilon_\alpha = 0.00035$ and $T_\alpha = 1$, $\epsilon_\beta = 0.00035$ and $T_\beta = 1.5$, $\epsilon_\text{ODIN} = 0$ and $T_\text{ODIN} = 1.3$, $\epsilon_\text{MHLNB} = 0.0002$ and $T_\text{MHLNB} = 1$, $\epsilon_\text{ENERGY} = 0$ and $T_\text{ENERGY} = 1$. In TBB for ODIN we report same results as in SR, since both methods coincide when $T=1$ and $\epsilon=0$.}
	\begin{center}
		%\begin{subtable}[h]{.5\textwidth}
			%
			\begin{small}
			\resizebox{0.7\textwidth}{!}{
				%	\makebox[\textwidth][c]{
						\begin{sc}
						\begin{tabular}{c|c|c|c|c|c}
								\toprule
							\multirow{2}{5em}{\textbf{DATASET}} & \multirow{2}{5em}{\textbf{METHOD}} & \multicolumn{2}{c}{\textbf{AUROC} $\%$} & \multicolumn{2}{|c}{\textbf{FRR $\%$ (95 $\%$ TRR) }}\Bstrut\\\cline{3-6}
								& & TBB & PBB & TBB & PBB\Tstrut\Bstrut\\
								\hline
								\midrule
								\multirow{5}{5em}{\parbox[t][][c]{3cm}{
 CIFAR10\\\textnormal{Acc.} $95\%$}}  
& $D_\alpha$ & \textbf{94} & \textbf{95.2} & \textbf{17.9} & 13.9\Bstrut\\\cline{2-6}
& $D_\beta$  &   68.5 & 94.8 & 18.6 & \textbf{13.4}\Tstrut\Bstrut\\\cline{2-6}
& ODIN       & 93.8 & 94.2 & 18.2 & 18.4\Tstrut\Bstrut\\\cline{2-6}
& SR         & 93.8 & - & 18.2 & -\Tstrut\Bstrut\\\cline{2-6}
& MHLNB      &   92.2  & 84.4 & 30.8 & 44.6\Tstrut\Bstrut\\\cline{2-6}
& ENERGY      &   -  & 91.1 & - & 34.7\Tstrut\\
								\midrule
								\multirow{5}{5em}{\parbox[t][][c]{3cm}{
 CIFAR100\\\textnormal{Acc.} $78\%$}} 
& $D_\alpha$ & \textbf{87} &\textbf{88.2} & 40.6 & \textbf{35.7}\Bstrut\\\cline{2-6}
& $D_\beta$  &   84.2  & 87.4 & 40.6 & 36.7\Tstrut\Bstrut\\\cline{2-6}
& ODIN       &  86.9 & 87.1 & 40.5 & 40.7\Tstrut\Bstrut\\\cline{2-6}
& SR         &  86.9 & - & \textbf{40.5} &-\Tstrut\Bstrut\\\cline{2-6}
& MHLNB      &   82.6   & 50 & 66.7 & 94\Tstrut\Bstrut\\\cline{2-6}
& ENERGY      &   -  & 78.7 & - & 65.4\Tstrut\\
								\midrule
								\multirow{5}{5em}{\parbox[t][][c]{3cm}{
 Tiny\\ImageNet\\\textnormal{Acc.} $63\%$}}   
& $D_\alpha$ & \textbf{84.9} &\textbf{86.1} & \textbf{45.8} &  \textbf{43.3} \Bstrut\\\cline{2-6}
& $D_\beta$  &  \textbf{84.9}  & 85.3 & \textbf{45.8} & 45.1 \Tstrut\Bstrut\\\cline{2-6}
& ODIN       & \textbf{84.9} & 84.9 & \textbf{45.8} & 45.3\Tstrut\Bstrut\\\cline{2-6}
& SR         & \textbf{84.9} & - & \textbf{45.8} & -\Tstrut\Bstrut\\\cline{2-6}
& MHLNB      &    78.4 & 59 & 82.3&  86\Tstrut\Bstrut\\\cline{2-6}
& ENERGY      &   -  & 78.2 & - & 63.7\Tstrut\\
\midrule
\multirow{5}{5em}{\parbox[t][][c]{3cm}{ SVHN\\ \textnormal{Acc.} $96\%$}} 
& $D_\alpha$ & \textbf{92.3}  & \textbf{93} & \textbf{38.6} & \textbf{36.6}\Bstrut\\\cline{2-6}
& $D_\beta$  &  92.2  &  92.8 & 39.7 & 38.4\Tstrut\Bstrut\\\cline{2-6}
& ODIN       & \textbf{92.3}  & 92.3 &  \textbf{38.6} & 40.7  \Tstrut\Bstrut\\\cline{2-6}
& SR         & \textbf{92.3} &  - & \textbf{38.6}  & - \Tstrut\Bstrut\\\cline{2-6}
& MHLNB      &  87.3    & 88 & 85.8 & 54.7\Tstrut\Bstrut\\\cline{2-6}
& ENERGY      &   -  & 88.9 & - & 49.4\Tstrut\\

								\bottomrule
							\end{tabular}
						\end{sc}
				%	}
				}
			\end{small}
	%	\end{subtable}
		\end{center}
	\label{tab:best_aurocs}
\end{table}

==> rebuttal/table_ood.tex <==
\begin{table}[!htb]
\centering
	\caption{The results are in terms of \textit{mean / standard deviation}.
	}
	\begin{center}
		\begin{small}
		\resizebox{1.1\textwidth}{!}{
		\begin{sc}
			\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
				\toprule
				\multirow{2}{5em}{\centering\textbf{DATASET-In}} & \multirow{2}{5em}{\centering\textbf{DATASET-Out}} & \multicolumn{4}{c}{\textbf{AUROC $\%$}} & \multicolumn{4}{|c}{\textbf{FRR $\%$ (95 $\%$ TRR)}}\Bstrut\\\cline{3-10}
								& & $D_\alpha$ & $D_\beta$ & ODIN & ENERGY & $D_\alpha$ & $D_\beta$ & ODIN & ENERGY\Tstrut\\
								\hline
								\midrule
								\multirow{2}{5em}{\parbox[t][][t]{1cm}{\centering
 CIFAR10\\$\clubsuit$}}  
& iSUN & \textbf{95.4} / 0.1  & 95.1 / 0.1  & 94.6 / 0.1  & 92.4 / 0 &  14 / 0.5 &  \textbf{13.5} / 0.4 &  17.2 / 0.3 &  32.2 / 0.1\Bstrut\\\cline{2-10}
& Tiny (res) & \textbf{95.2} / 0.1  & 94.9 / 0  & 94.6 / 0.1  & 92.3 / 0.1  & \textbf{14} / 0.4 &  \textbf{14} / 0.5 &  17.8 / 0.4 &  32.2 / 0.1\Tstrut\Bstrut\\
\midrule
\multirow{2}{5em}{\parbox[t][][t]{1cm}{\centering
 CIFAR10\\$\diamondsuit$}}  
& iSUN  & \textbf{95.5} / 0.1  & 95.3 / 0.1  & 94.9 / 0.1 & 92.9 / 0 & 14.4 / 0.6 &  \textbf{13.4} / 0.2 &  16.8 / 0.5 & 27 / 1 \Bstrut\\\cline{2-10}
& Tiny (res) & \textbf{95.4} / 0.1  & 95 / 0.1  & 94.8 / 0.1  & 92.8 / 0 &  15 / 0.1 &  1\textbf{4.8} / 0.7 &  17 / 0.5 & 28.8 / 1.9\Tstrut\Bstrut\\
\midrule
\multirow{2}{5em}{\parbox[t][][t]{1cm}{\centering
 CIFAR10\\$\spadesuit$}}  
& iSUN  &  \textbf{95.6} / 0.1  & \textbf{95.6} / 0  & 95.4 / 0 & 93.6 / 0.1 &  15.1 / 0.1 &  \textbf{13.6} / 0.5 &  16.1 / 0.2 & 25.1 / 0.2 \Bstrut\\\cline{2-10}
& Tiny (res) &  \textbf{95.5} / 0.1  & 95.2 / 0.1  & 95.1 / 0.1  & 93.5 / 0 & \textbf{14.7} / 0.3 &  14.8 / 0.5 &  17.1 / 0.4 & 25.6 / 0.3\Tstrut\Bstrut\\
\bottomrule
\end{tabular}
		\end{sc}
		}
	\end{small}
\end{center}
\label{tab:ood_main}
\end{table}

==> tables/alphas.tex <==
\begin{table}[t]
\caption{Optimization of parameter $\alpha$ for function $\widehat{\fun{g}}$, CIFAR10. $\alpha\in\{2, 3, 4, 5, 6\}$. }
\label{table:alpha}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
T & $\bm{\alpha=2}$ & $\alpha=3$ & $\alpha=4$ & $\alpha=5$ &$\alpha=6$\\
\midrule
1    & \textbf{0.88739} & 0.65856 & 0.66186 & 0.66537 & 0.66943\\
1.5  & 0.93200 & 0.93339 & 0.93514 & 0.93590 & \textbf{0.93646}\\
2    & 0.94190 & \textbf{0.94237} & 0.94206 & 0.94189 & 0.94170\\
2.5  & 0.94067 & 0.94094 & 0.94094 & \textbf{0.94095} & 0.94062\\
3    & 0.93797 & 0.93935 & \textbf{0.93988} & 0.93973 & 0.93944\\
4    & 0.93166 & 0.93474 & 0.935670 & 0.\textbf{93602} & 0.93509\\
5    & 0.92468 & 0.92980 & \textbf{0.93115} & 0.92926 & 0.92849\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/aurocs_amazon.tex <==
\begin{table*}
	\caption{AUROCs for AmazonFashion, AmazonSoftware and IMDb for $T = 1$ and $\epsilon = 0$.}
	\vskip 0.15in
	\begin{center}
		\begin{small}
			\begin{sc}
				\resizebox{0.80\textwidth}{!}{
				\makebox[\textwidth][c]{
					\begin{tabular}{c|cccc|cccc|cccc}
						\toprule
						&\multicolumn{4}{c|}{AmazonFashion} & \multicolumn{4}{c|}{AmazonSoftware} & \multicolumn{4}{c}{IMDb}\\
						\midrule
						T & $\widehat{Pe}$ & DOCTOR & Odin  & SR & $\widehat{Pe}$ & DOCTOR & Odin & SR & $\widehat{Pe}$ & DOCTOR & Odin  & SR\\
						& & & ($\epsilon=0$) & &  & &($\epsilon=0$) & & & &($\epsilon=0$) &\\ 
						\midrule
						1   & 0.89717 & \textbf{0.89721}  & 0.87447 & 0.87447 & 0.68796 & \textbf{0.68800} & 0.67304 & 0.67304 & 0.83712 & \textbf{0.84156} & 0.83708& 0.83708\\
						\bottomrule
					\end{tabular}%
				}
			}
			\end{sc}
		\end{small}
	\end{center}
	\label{table:aurocs_amazon}
\end{table*}

==> tables/odin_eps.tex <==
\begin{table}[!htb]
	\caption{\textcolor{red}{Change table:ODIN: AUROCs for $T=1000$, $0 \leq \epsilon \leq 0.004$. The bold values correspond to the maximum AUROCs.}}
	%\vskip 0.05in
    \begin{center}
        %\begin{subtable}[h]{0.4\textwidth}
		    %\centering
			\begin{small}
				\resizebox{.3\textwidth}{!}{
			%		\makebox[\textwidth][c]{
					    \begin{sc}
						    \begin{tabular}{c|cc}
						    \toprule
						    &\multicolumn{2}{c}{\textbf{AUROC $\%$}}\\
						    \hline
						    \midrule
						    $\epsilon$    & TinyImagenet &   SVHN\\
						    \midrule
					        0              & 78.7 & 88.9\\
						    0.0002         & 78.7 & \textbf{89.1}\\
						    0.0004         & 78.6 & 88.8\\
						    0.0006         & 78.6 & 88.5\\
						    0.0008         & 78.7 & 88.1\\
						    0.001 & \textbf{78.8} & 87.8\\
						    0.0012         & 78.6 & 87.4\\
						    0.0014         & 78.5 & 87.1\\
						    0.0016         & 78.5 & 86.7\\
						    0.0018         & 78.4 & 86.4\\
						    0.002          & 78.3 & 86\\
						    0.0022         & 78.3 & 85.6\\
						    0.0024         & 78.3 & 85.3\\
						    0.0026         & 78.3 & 85.3\\
						    0.0028         & 78.2 & 84.7\\
						    0.003          & 78 & 84.4\\
						    0.0032         & 78 & 84\\
						    0.0034         & 78 & 83.8\\
						    0.0036         & 78 & 83.6\\
						    0.0038         & 78 & 83.3\\
						    0.004          & 78 & 83\\ 
						    \bottomrule
					        \end{tabular}
					    \end{sc}
				%	}
				}
			\end{small}
	%	\end{subtable}
	\end{center}
\label{tab:best_odin}
\vskip -0.1in
\end{table}

==> tables/rebuttal.tex <==
% !TEX root = ../rebuttal_main.tex
\begin{table}[!htb]
	\caption{Best AUROCs obtained via DOCTOR, ODIN and SR and Mahalanobis for image datasets. Values in bold correspond to the maximum AUROCs. In \textit{totally black box} only the last layer of the network is available, hence no input pre-processing can be performed. In \textit{partially black box} we suppose is possible to perturb the input as in~\cref{eq:perturb_alpha},~\cref{eq:perturb_odin} and~\cref{eq:perturb_mahalanobis} for $D_\alpha$, ODIN and MHLNB, respectively. The perturbation values are: $\epsilon_{\alpha}=0.00035$ for $D_\alpha$; $\epsilon_{\text{ODIN}}$ as in \cite{LiangLS2018ICLR} for ODIN; $\epsilon_{\text{MHLNB}}=0.0002$ for MHLNB.}
	\begin{center}
		\begin{small}
			\resizebox{.7\textwidth}{!}{
			\begin{sc}
				\begin{tabular}{c|c|c|c|c|c|c|c}
				    \toprule
					\textbf{DATASET} & \textbf{METHOD} & \textbf{TBB $\%$} & \textbf{PBB $\%$}&\textbf{DATASET} & \textbf{METHOD} & \textbf{TBB $\%$} & \textbf{PBB $\%$}\\
					\hline
					\midrule
					\multirow{4}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR10\\\textnormal{Accuracy} $95\%$}}  & $D_\alpha$ & \textbf{94.3} & \textbf{95.2} & \multirow{4}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR100\\\textnormal{Accuracy} $78\%$}} & $D_\alpha$ & \textbf{87} & \textbf{88.2}\\\cmidrule{2-4}\cmidrule{6-8}
& ODIN       & - & 87.4& & ODIN & - & 78\\ \cmidrule{6-8}\cmidrule{2-4}
& SR         & 93.8 & - & & SR &  86.9 & -\\\cmidrule{6-8}\cmidrule{2-4}
& MHLNB  & 84.2 & 84.4 & & MHLNB  & 50 & 50\\
\midrule

\multirow{4}{*}{\parbox[t][][c]{3cm}{\centering
 TinyImageNet\\\textnormal{Accuracy} $63\%$}}   & $D_\alpha$ & \textbf{84.9} & \textbf{86} & \multirow{4}{*}{\parbox[t][][c]{3cm}{\centering
 SVHN\\ \textnormal{Accuracy} $96\%$}} & $D_\alpha$ & \textbf{92.3} & \textbf{93}\\\cmidrule{6-8}\cmidrule{2-4}
& ODIN       & - & 78.8 & & ODIN       & - & 89.1\\ \cmidrule{6-8} \cmidrule{2-4}
& SR         & \textbf{84.9} & - & & SR         & \textbf{92.3} & -\\\cmidrule{6-8}\cmidrule{2-4}
& MHLNB  & 59 & 59 & & MHLNB  & 87.9 & 88\\
\bottomrule
				    \end{tabular}
			    \end{sc}
		    }
	    \end{small}
    \end{center}
\label{tab:best_aurocs_total}
\end{table}

==> tables/tab_alpha.tex <==
\begin{table}[!htb]
	\caption{$D_\alpha$ when perturbation as in~\eqref{eq:perturb_alpha} is applied. We have set $T$ to the values in the table and varied $\epsilon$ in $\{0,~0.0002,~0.00025,~0.0003,~0.00035,$ $~0.0004,~0.0006,~0.0008, 0.001,~0.0012,$ $0.0014,~0.0016,~0.0018,~0.002,~0.0022,$ $0.0024,~0.0026,~0.0028,~0.003,~0.0032$ $0.0034,~0.0036,~0.0038,~0.004\}$; $\epsilon^*$ denotes the $\epsilon$ with which the best AUROC is reached w.r.t. $T$.}
	\begin{center}
		\begin{small}
			\resizebox{.7\textwidth}{!}{
			\begin{sc}
				\begin{tabular}{c|c|c|c|c|c|c|c}
				    \toprule
					\textbf{DATASET} & \textbf{T} & \textbf{$\epsilon^*$} & \textbf{AUROC $\%$} & \textbf{DATASET} & \textbf{T} & \textbf{$\epsilon^*$} & \textbf{AUROC $\%$}\\ 
					\hline
					\midrule
					\multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR10\\\textnormal{Accuracy} $95\%$\\~\\\textnormal{Previous Best AUROC} $94.3\%$}}  
& \textbf{1} & \textbf{0.0003} & \textbf{95.4} 
& \multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 TinyImageNet\\\textnormal{Accuracy} $63\%$\\~\\\textnormal{Previous Best AUROC} $84.9\%$}} 
& \textbf{1} & \textbf{0.0006} & \textbf{86.8} \\ \cmidrule{2-4}\cmidrule{6-8}
& 1.1 & 0.0003 & 95.4 & & 1.1 & 0.0006 & 86.5 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.2 & 0.0003 & 95.4 & & 1.2 & 0.0006 & 86.3  \\\cmidrule{2-4}\cmidrule{6-8}
& 1.3 & 0.0003 & 95.3 & & 1.3 & 0.0008 & 85.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.4 & 0.0003 & 95.3 & & 1.4 & 0.0008 & 85.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.5 & 0.0003 & 95.3 & & 1.5 & 0.0008 & 85 \\\cmidrule{2-4}\cmidrule{6-8}
& 2 & 0.0003 & 95 & & 2 & 0.0008 & 82.7 \\\cmidrule{2-4}\cmidrule{6-8}
& 2.5 & 0.0002 & 94.6 & & 2.5 & 0 & 80.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 3 & 0.0003 & 94 & & 3 & 0 & 79.2 \\\cmidrule{2-4}\cmidrule{6-8}
& 100 & 0.0014 & 83.6 & & 100 & 0.0016 & 51.2 \\\cmidrule{2-4}\cmidrule{6-8}
& 1000 & 0.0016 & 83.1 & & 1000 & 0.0016 & 50.8\\
\midrule
\multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR100\\\textnormal{Accuracy} $78\%$\\~\\\textnormal{Previous Best AUROC} $87\%$}}
& \textbf{1} & \textbf{0.00035} & \textbf{88.2} & \multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 SVHN\\\textnormal{Accuracy} $96\%$\\~\\\textnormal{Previous Best AUROC} $92.3\%$}}  
& \textbf{1} & \textbf{0.001} & \textbf{93.9} \\ 
\cmidrule{2-4}\cmidrule{6-8}
& 1.1 & 0.00035 & 88.2 & & 1.1 & 0.001 & 93.8\\\cmidrule{2-4}\cmidrule{6-8}
& 1.2 & 0.00035 & 87.9 & & 1.2 & 0.001 & 93.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.3 & 0.0004 & 87.8 & & 1.3 & 0.001 & 93.7  \\\cmidrule{2-4}\cmidrule{6-8}
& 1.4 & 0.0004 & 87.5 & & 1.4 & 0.001 & 93.6 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.5 & 0.0004 & 87.2 & & 1.5 & 0.001 & 93.5 \\\cmidrule{2-4}\cmidrule{6-8}
& 2 & 0 & 85.6 & & 2 & 0.0012 & 92.7\\\cmidrule{2-4}\cmidrule{6-8}
& 2.5 & 0 & 84.1 & & 2.5 & 0.001 & 92  \\\cmidrule{2-4}\cmidrule{6-8}
& 3 & 0 & 82.6 & & 3 & 0.001 & 91.3 \\\cmidrule{2-4}\cmidrule{6-8}
& 100 & 0.0036 & 69.4 & & 100 & 0.0034 & 84.4 \\\cmidrule{2-4}\cmidrule{6-8}
& 1000 & 0.0036 & 68.7 & & 1000 & 0.0034 & 84\\
\bottomrule
				    \end{tabular}
			    \end{sc}
		    }
	    \end{small}
    \end{center}
\label{tab:alpha}
\end{table}

==> tables/tab_cifar10.tex <==
\begin{table*}[!htb]
	\caption{Summative results: CIFAR10}
	\begin{center}
		\begin{small}
			\resizebox{.9\textwidth}{!}{
			\begin{sc}
			\begin{tabular}{cl|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
            \toprule
            \multicolumn{26}{c}{\textbf{AUROC $\%$}}\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{2}{2em}{\centering T} & \multirow{2}{2em}{\centering Method} & \multicolumn{24}{c}{$\epsilon$}\\
            \cline{3-26}
            %\cmidrule[\heavyrulewidth]{3-26}
            && 0 & .0002 & .00025 & .0003 & .00035 & .0004 & .0006 & .0008 & .001 & .0012 & .0014 & .0016 & .0018 &
                .002 & .0022 & .0024 & .0026 & .0028 & .003 & .0032 & .0034 & .0036 & .0038 & .004\Tstrut\Bstrut\\
            \hline
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{4}{2em}{\centering 1} & $D_\alpha$ & 94 & 95.2 & 95.2 & 95.4 & 95.2 & 95 & 93.2 & 91 & 87.8 & 84.9 & 82.1 & 79.3 & 77.2 & 75 & 73.1 & 70.9 & 68.8 & 68 & 67 & 66.4 & 65.5 & 65.5 & 65.1 & 65 \Bstrut\\\cline{2-26} 
            & $D_\beta$ & 68.5 & 70.3 & 70.3 & 70.4 & 70.1 & 69.8 & 67.6 & 64.7 & 60.7 & 57 & 53.5 & 49.8 & 46.9 & 43.8 & 40.9 & 38 & 35.3 & 33.4 & 31.3 & 29.8 & 28.2 & 27.1 & 25.9 & 24.9  \Tstrut\Bstrut\\ \cline{2-26}
            & SR & 93.8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - &-\Tstrut\Bstrut\\\cline{2-26}
            & ODIN  & 93.8 & 92.8 & 92.7 & 92.1 & 91.6 & 90.8 & 88.3 & 83.8 & 80.5 & 76.2 & 73.1 & 69.5 & 66.4 & 64 & 62.1 & 60.6 & 59.2 & 58.4 & 57.8 & 57.6 & 57.7 & 57.3 & 57.2 & 56.7 \Tstrut\Bstrut\\\cline{2-26} 
            & MHLNB & 84.2 & 84.4 & 84.2 & 83.8 & 83.5 & 83.1 & 80 & 76.6 & 72.7 & 69 & 65.8 & 62.9 & 60.1 & 57.7 & 55.8 & 53.6 & 51.8 & 50.4 & 49.1 & 47.9 & 46.8 & 45.9 & 45.1 & 44.3\Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{3}{2em}{\centering 1.1} & $D_\alpha$ & 94.1 & 95.2 & 95.2 & 95.4 & 95.1 & 95 & 93.3 & 91.2 & 88 & 85 & 82.4 & 79.2 & 77 & 74.8 & 72.5 & 70 & 67.5 & 66.3 & 65 & 63.7 & 62.7 & 62 & 61.4 & 61.1 \Bstrut\\\cline{2-26}  
            & $D_\beta$ & 78.5 & 80.1 & 80.1 & 80.3 & 79.9 & 79.6 & 77.6 & 75.1 & 71.4 & 68 & 64.8 & 61.2 & 58.4 & 55.5 & 52.7 & 49.5 & 46.7 & 44.8 & 42.7 & 40.9 & 39.3 & 38 & 36.7 & 35.7\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94.1 & 93.6 & 93.2 & 92.9 & 92.7 & 92.5 & 90.5 & 87.6 & 83.8 & 80.6 & 76.8 & 74.7 & 71.3 & 68.5 & 66.9 & 65.1 & 63.3 & 62.2 & 61.1 & 60.9 & 60.4 & 59.7 & 59.2 & 58.9\Tstrut\\
            %& MHLNB & \Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.2} & $D_\alpha$ & 94.1 & 95.2 & 95.2 & 95.4 & 95.2 & 95 & 93.4 & 91.2 & 88 & 85.2 & 82.6 & 79.5 &  77.2 & 75 & 72.5 & 69.8 & 67.2 & 65.6 & 64 & 62.7 & 61.2 & 60.7 & 59.3 & 58.9 \Bstrut\\\cline{2-26} 
            & $D_\beta$ & 86 & 87.4 & 87.4 & 87.6 & 87.3 & 87 & 85.2 & 82.8 & 79.4 & 76.2 & 73.3 & 69.8 & 67.2 & 64.7 & 61.9 & 59 & 56 & 54.1 & 52.2 & 50.4 & 48.8 & 47.8 & 46.2 & 45.1\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94.1 & 93.9 & 93.7 & 93.5 & 93.4 & 93 & 91.7 & 90 & 87.2 & 84.1 & 81.8 & 78.8 & 75.7 & 73.1 & 70.9 & 69.2 & 67.5 & 66.1 & 65.4 & 63.9 & 63.3 & 62.9 & 62.2 & 61.5\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{4}{2em}{\centering 1.3} & $D_\alpha$ & 94.2 & 95.2 &   95.2 & 95.4 & 95.3 & 95 & 93.4 & 91.3 & 88.3 & 85.5 & 82.9 & 79.9 & 77.5 & 75.2 & 72.8 & 70 & 67.4 & 65.9 & 64.1 & 62.5 & 61 & 60.2 & 58.9 & 58 \Bstrut\\\cline{2-26}
             & $D_\beta$ & 90.6 & 91.8 & 91.8 & 92 & 91.7 & 91.5 & 89.8 & 87.5 & 84.3 & 81.3 & 78.4 & 75.3 & 72.9 & 70.5 & 67.9 & 65 & 62.2 & 60.5 & 58.6 & 56.9 & 55.1 & 54.2 & 52.7 & 51.6 \Tstrut\Bstrut\\ \cline{2-26}
            & ODIN & 94.2 & 94 & 93.9 & 93.8 & 93.6 & 93.6 & 92.7 & 91.2 & 89.6 & 87.4 & 85.1 & 83 & 79.7 & 77.6 & 76.1 & 73.3 & 71.5 & 70.4 & 68.5 & 67.8 & 67.1 & 66.3 & 65.3 & 64.6 \Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.4} & $D_\alpha$ & 94.2 & 95.2 & 95.2 & 95.4 & 95.2 & 95 & 93.4 & 91.4 & 88.5 & 85.7 & 83.1 & 80.2 & 77.9 & 75.5 & 73.1 & 70.5 & 68 & 66.3 & 64.5 & 62.8 & 61.3 & 60.4 & 59 & 58 \Bstrut\\\cline{2-26} 
             & $D_\beta$ & 92.9 & 93.9 & 94 & 94.1 & 93.9 & 93.6 & 92.1 & 89.9 & 86.7 & 83.8 & 81.2 & 78.2 & 75.9 & 73.5 & 71 & 68.4 & 65.8 & 64.1 & 62.2 & 60.5 & 58.8 & 57.9 & 56.5 & 55.4\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94.2 & 94 & 93.9 & 93.8 & 93.7 & 93.6 & 93.3 & 92.1 & 90.8 & 89.2 & 87.8 & 86 & 83.7 & 81.4 & 79.1 & 77.5 & 76.3 & 74.1 & 73.2 & 72 & 71.2 & 70.1 & 69.1 & 68.1 \Tstrut\\ 
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 1.5} & $D_\alpha$ & 94.3 & 95.1 & 95.2 & 95.3 & 95.2 & 94.9 & 93.4 & 91.5 & 88.7 & 86 & 83.4 & 80.4 & 78.2 & 75.9 & 73.5 & 70.9 & 68.3 & 66.8 & 65 & 63.2 & 61.8 & 60.7 & 59.6 & 58.3 \Bstrut\\\cline{2-26} 
            & $D_\beta$ & 93.7 & 94.8 & 94.8 & 95 & 94.8 & 94.5 & 92.9 & 90.8 & 87.8 & 84.9 & 82.3 & 79.4 & 77.1 & 74.9 & 72.4 & 69.8 & 67.2 & 65.6 & 63.8 & 62.1 & 60.6 & 59.6 & 58.3 & 57.0\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN & 94.2 & 94 & 93.9 & 93.9 & 93.8 & 93.7 & 93.2 & 92.6 & 91.6 & 90.4 & 89.1 & 87.9 & 86.3 & 84.4 & 82.9 & 81.1 & 79.2 & 77.9 & 76.9 & 75.7 & 74.3 & 73.2 & 72.7 & 71.8 \Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2} & $D_\alpha$ & 94.2 & 95 & 95 & 95 & 95 & 94.6 & 93.4 & 91.6 & 89.2 & 86.7 & 84.4 & 81.8 & 79.4 & 77.4 & 75.3 & 72.6 & 70.5 & 68.7 & 67.2 & 65.8 & 64 & 62.8 & 61.8 & 60.5 \Bstrut\\\cline{2-26}  
            & $D_\beta$ & 94.2 & 95.1 & 95.2 & 95.3 & 95.1 & 94.7 & 93.2 & 91.2 & 88.5 & 85.7 & 83.4 & 80.5 & 78.2 & 76.2 & 74.2 & 71.5 & 69.4 & 67.5 & 66.2 & 64.7 & 62.9 & 61.8 & 60.8 & 59.7\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94.2 & 93.9 & 93.9 & 93.8 & 93.7 & 93.6 & 93.1 & 92.6 & 92.1 & 91.6 & 91 & 90.3 & 89.7 & 89.1 & 88.6 & 88 & 87.4 & 87 & 86.4 & 85.7 & 85.4 & 84.8 & 84.5 & 84.0 \Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2.5} & $D_\alpha$ & 94 & 94.6 & 94.5 & 94.5 & 94.5 & 94.5 & 93.2 & 91.9 & 89.7 & 87.3 & 85.1 & 82.7 & 80.4 & 78.7 & 76.9 & 74.3 & 72.3 & 70.8 & 69.2 & 67.9 & 66.3 & 65 & 63.9 & 62.8 \Bstrut\\\cline{2-26} 
            & $D_\beta$ & 94.1 & 95 & 95 & 95.1 & 95 & 94.6 & 93.1 & 91.1 & 88.6 & 85.9 & 83.7 & 80.9 & 78.5 & 76.9 & 75.2 & 72.5 & 70.5 & 68.9 & 67.5 & 66.2 & 64.6 & 63.4 & 62.3 & 61.3\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94.1 & 93.8 & 93.8 & 93.7 & 93.6 & 93.4 & 93 & 92.4 & 91.9 & 91.3 & 90.7 & 90.1 & 89.5 & 89 & 88.4 & 88 & 87.5 & 87 & 86.6 & 86.3 & 85.9 & 85.5 & 85.2 & 84.8 \Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 3} & $D_\alpha$ & 93.8 & 94 & 94 & 94 & 94 & 94 & 92.8 & 91.4 & 89.6 & 87.5 & 85.5 & 83.3 & 81.2 & 79.4 & 77.8 & 75.7 & 73.5 & 72 & 70.5 & 69.3 & 67.9 & 66.7 & 65.6 & 64.3 \Bstrut\\\cline{2-26}
            & $D_\beta$ & 94 & 94.8 & 94.8 & 94.8 & 94.7 & 94.3 & 92.8 & 91 & 88.4 & 86 & 83.6 & 81.2 & 79 & 77.3 & 75.8 & 73.4 & 71.1 & 69.9 & 68.3 & 67.3 & 65.8 & 64.7 & 63.7 & 62.5\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 94 & 93.7 & 93.6 & 93.5 & 93.4 & 93.3 & 92.8 & 92.3 & 91.7 & 91.1 & 90.5 & 89.9 & 89.3 & 88.7 & 88.2 & 87.7 & 87.2 & 86.8 & 86.4 & 86 & 85.6 & 85.3 & 84.9 & 84.5\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 100} & $D_\alpha$ & 82 & 82.1 & 82.1 & 82 & 82 & 82 & 82.5 & 83 & 83 & 83.1 & 83.7 & 83.7 & 83.6 & 83.3 & 82.5 & 82 & 81 & 80.4 & 79.7 & 79.2 & 78.7 & 78 & 77.3 & 76.7  \Bstrut\\\cline{2-26}  
            & $D_\beta$ & 91.5 & 91.4 & 91.5 & 91.5 & 91.5 & 91.4 & 90.4 & 89.2 & 87.6 & 86.2 & 84.8 & 83.4 & 81.9 & 80.5 & 79.5 & 78.7 & 77.2 & 76.2 & 75.3 & 74.5 & 73.4 & 72.7 & 71.8 & 70.7\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 91.5 & 91.1 & 91 & 90.9 & 90.8 & 90.6 & 90.1 & 89.6 & 89 & 88.4 & 87.7 & 87.1 & 86.4 & 85.8 & 85.3 & 84.8 & 84.3 & 83.8 & 83.3 & 82.9 & 82.5 & 82.1 & 81.7 & 81.4\Tstrut\\
            \midrule
             \multirow{3}{2em}{\centering 1000} & $D_\alpha$ & 80.3 & 80.5 & 80.5 & 80.3 & 80.4 & 80.4 & 81 & 81.9 & 82 & 82 & 82.5 & 83.2 & 83 & 83 & 82.7 & 82.3 & 81.5 & 80.7 & 80 & 79.3 & 78.7 & 78.1 & 77.4 & 76.7  \Bstrut\\\cline{2-26} 
            & $D_\beta$ & 91.4 & 91.3 & 91.3 & 91.4 & 91.4 & 91.4 & 90.2 & 89.1 & 87.6 & 86.2 & 84.7 & 83.5 & 82 & 80.5 & 79.5 & 78.7 & 77.3 & 76.3 & 75.4 & 74.6 & 73.5 & 72.8 & 71.9 & 70.7\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 91.2 & 90.9 & 90.7 & 90.6 & 90.5 & 90.4 & 90 & 89.3 & 88.7 & 88.1 & 87.4 & 87 & 86.2 & 85.5 & 85 & 84.6 & 84.1 & 83.6 & 83.1 & 82.8 & 82.2 & 82 & 81.6 & 81.3\Tstrut\\
            %& MHLNB &\\
            \bottomrule
        \end{tabular}
        \end{sc}
		 }
	    \end{small}
    \end{center}
\label{tab:cifar10}
\end{table*}

==> tables/tab_cifar100.tex <==
\begin{table*}[!htb]
	\caption{Summative results: CIFAR100}
	\begin{center}
		\begin{small}
			\resizebox{.9\textwidth}{!}{
			\begin{sc}
			\begin{tabular}{cl|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
            \toprule
            \multicolumn{26}{c}{\textbf{AUROC $\%$}}\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{2}{2em}{\centering T} & \multirow{2}{2em}{\centering Method} & \multicolumn{24}{c}{$\epsilon$}\\
            \cline{3-26}
            %\cmidrule[\heavyrulewidth]{3-26}
            && 0 & .0002 & .00025 & .0003 & .00035 & .0004 & .0006 & .0008 & .001 & .0012 & .0014 & .0016 & .0018 &
                .002 & .0022 & .0024 & .0026 & .0028 & .003 & .0032 & .0034 & .0036 & .0038 & .004\Tstrut\Bstrut\\
            \hline
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{4}{2em}{\centering 1} & $D_\alpha$   & 87 & 87.9 & 88.2 & 88.2 & 88.2 & 88.1 & 87.5 & 85.6 & 83.1 & 81.1 & 78.9 & 76.7 & 74.7 & 73.1 & 72 & 70.6 & 69 & 67.7 & 66.5 & 65.8 & 65.2 & 64.7 & 63.9 & 63.3\Bstrut\\\cline{2-26}
            & $D_\beta$   & 84.2 & 84.7 & 85.1 & 85 & 84.6 & 84.2 & 83.1 & 80.5 & 77.5 & 75.1 & 72.5 & 70 & 67.8 & 65.9 & 64.6 & 62.9 & 61.3 & 59.8 & 58.4 & 57.6 & 57 & 56.4 & 55.6 & 54.9\Tstrut\Bstrut\\\cline{2-26}
            & SR & 86.9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - &-\Tstrut\Bstrut\\\cline{2-26}
            & ODIN   & 86.9 & 86.8 & 86.8 & 86.7 & 86.7 & 86.6 & 86.2 & 85.9 & 85.4 & 85 & 84.5 & 84 & 83.4 & 82.8 & 82.3 & 81.6 & 81 & 80.3 & 79.8 & 79.1 & 78.3 & 77.8 & 77.4 & 77.0\Tstrut\Bstrut\\\cline{2-26} 
            & MHLNB & 49.1 & 49 & 48.8 & 48.7 & 48.3 & 48.1 & 47.1 & 46 & 45.1 & 44.5 & 44.1 & 43.7 & 43.2 & 42.9 & 42.6 & 42.4 & 42.2 & 41.9 & 41.6 & 41.2 & 41.2 & 41.2 & 41.2 & 41.2 \Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{3}{2em}{\centering 1.1} & $D_\alpha$   & 87.1 & 87.8 & 87.9 & 88.2 & 88.2 & 88 & 87.7 & 85.9 & 83.8 & 81.9 & 79.7 & 77.7 & 76.1 & 74.6 & 73.4 & 71.9 & 70.5 & 69.2 & 68 & 67 & 66.3 & 65.5 & 64.7 & 64.1\Bstrut\\\cline{2-26}
& $D_\beta$   & 85.5 & 86 & 86.4 & 86.3 & 86 & 85.7 & 84.7 & 82.3 & 79.6 & 77.3 & 74.9 & 72.7 & 70.8 & 69.1 & 67.8 & 66.3 & 64.8 & 63.3 & 62.1 & 61.2 & 60.6 & 59.8 & 59 & 58.4\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 87 & 86.9 & 86.9 & 86.8 & 86.8 & 86.7 & 86.4 & 86 & 85.7 & 85.3 & 84.9 & 84.5 & 84 & 83.5 & 83 & 82.5 & 82 & 81.5 & 81 & 80.5 & 80.1 & 79.5 & 79.1 & 78.7\Tstrut\\
            %& MHLNB & \Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.2} & $D_\alpha$   & 87 & 87.6 & 87.7 & 88 & 88 & 87.8 & 87.7 & 86.2 & 84.3 & 82.6 & 80.5 & 78.8 & 77.1 & 75.8 & 74.4 & 73.2 & 71.6 & 70.4 & 69.1 & 67.8 & 67.3 & 66.6 & 66 & 65.2\Bstrut\\\cline{2-26}
& $D_\beta$   & 86.3 & 86.8 & 87.1 & 87 & 86.8 & 86.5 & 85.7 & 83.5 & 80.9 & 78.9 & 76.5 & 74.5 & 72.7 & 71.3 & 69.9 & 68.7 & 67.1 & 66 & 64.6 & 63.3 & 63.1 & 62.6 & 62 & 61.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 87.1 & 87 & 86.9 & 86.9 & 86.8 & 86.8 & 86.5 & 86.1 & 85.8 & 85.5 & 85.1 & 84.7 & 84.4 & 84 & 83.6 & 83.1 & 82.7 & 82.2 & 81.8 & 81.5 & 81 & 80.5 & 80.1 & 79.8\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{4}{2em}{\centering 1.3} & $D_\alpha$   & 87 & 87.4 & 87.5 & 87.7 & 87.7 & 87.8 & 87.5 & 86.3 & 84.6 & 83 & 81.2 & 79.5 & 77.9 & 76.6 & 75.5 & 74.2 & 72.7 & 71.5 & 70.2 & 69 & 68.4 & 68 & 67.2 & 66.5\Bstrut\\\cline{2-26}
& $D_\beta$   & 86.6 & 87.1 & 87.4 & 87.4 & 87.2 & 86.9 & 86 & 84 & 81.6 & 79.9 & 77.7 & 75.6 & 74 & 72.6 & 71.3 & 70.1 & 68.7 & 67.5 & 66.2 & 65.1 & 64.9 & 64.5 & 63.7 & 63.0\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 87.1 & 87 & 87 & 86.9 & 86.9 & 86.8 & 86.5 & 86.2 & 85.9 & 85.6 & 85.2 & 84.9 & 84.5 & 84.1 & 83.7 & 83.3 & 83 & 82.6 & 82.2 & 81.8 & 81.4 & 80.9 & 80.6 & 80.3\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.4} & $D_\alpha$   & 86.9 & 87 & 87.3 & 87.4 & 87.5 & 87.5 & 87.2 & 86.4 & 84.8 & 83.4 & 81.8 & 80.2 & 78.8 & 77.7 & 76.2 & 75 & 73.7 & 72.5 & 71.3 & 70.2 & 69.5 & 68.9 & 68.2 & 67.5\Bstrut\\\cline{2-26}
& $D_\beta$   & 86.8 & 87.2 & 87.5 & 87.6 & 87.3 & 87 & 86.2 & 84.4 & 82.2 & 80.6 & 78.6 & 76.6 & 74.9 & 73.6 & 72.4 & 71.3 & 69.8 & 68.6 & 67.4 & 66.6 & 66.1 & 65.6 & 64.9 & 64.4\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 87.1 & 87 & 87 & 86.9 & 86.9 & 86.8 & 86.5 & 86.2 & 85.9 & 85.6 & 85.3 & 85 & 84.6 & 84.2 & 83.9 & 83.5 & 83.2 & 82.8 & 82.4 & 82 & 81.7 & 81.3 & 80.9 & 80.7\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 1.5} & $D_\alpha$   & 86.8 & 86.8 & 87 & 87.1 & 87.2 & 87.2 & 87 & 86.4 & 85 & 83.7 & 82.1 & 80.7 & 79.4 & 78.2 & 77 & 75.9 & 74.4 & 73.2 & 72.1 & 71 & 70.4 & 69.8 & 69.3 & 68.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 86.8 & 87.2 & 87.4 & 87.6 & 87.4 & 87 & 86.2 & 84.6 & 82.5 & 80.8 & 79 & 77.2 & 75.7 & 74.3 & 73.3 & 72.1 & 70.7 & 69.3 & 68.4 & 67.4 & 67.2 & 66.5 & 66 & 65.4\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 87 & 87 & 86.9 & 86.9 & 86.8 & 86.8 & 86.5 & 86.2 & 85.9 & 85.7 & 85.4 & 85 & 84.7 & 84.3 & 84 & 83.6 & 83.3 & 82.9 & 82.5 & 82.2 & 81.8 & 81.5 & 81 & 80.8
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2} & $D_\alpha$   & 85.6 & 85.1 & 85.1 & 85.2 & 85.2 & 85.3 & 85.4 & 85 & 84.3 & 83.8 & 83 & 81.6 & 80.6 & 79.9 & 79.1 & 78 & 77.1 & 76.4 & 75.4 & 74.6 & 73.8 & 73.2 & 72.8 & 72.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 86.4 & 86.7 & 86.7 & 86.8 & 86.7 & 86.5 & 85.6 & 84.5 & 83 & 81.7 & 80.2 & 78.6 & 77.4 & 76.4 & 75.2 & 74.2 & 73.5 & 72.4 & 71.4 & 70.5 & 70 & 69.5 & 69.2 & 68.9\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 86.5 & 86.5 & 86.5 & 86.5 & 86.4 & 86.4 & 86.3 & 86 & 85.8 & 85.6 & 85.3 & 85 & 84.7 & 84.4 & 84 & 83.7 & 83.4 & 83 & 82.7 & 82.3 & 82 & 81.6 & 81.3 & 80.9
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2.5} & $D_\alpha$   & 84.2 & 83.5 & 83.3 & 83.3 & 83.2 & 83.2 & 83.7 & 83.3 & 82.9 & 82.5 & 82.2 & 81.4 & 80.9 & 80.5 & 79.6 & 78.9 & 78 & 77.6 & 76.9 & 76.1 & 75.2 & 74.9 & 74.5 & 74.0\Bstrut\\\cline{2-26}
& $D_\beta$   & 85.6 & 85.6 & 85.7 & 85.6 & 85.6 & 85.5 & 84.6 & 83.7 & 82.5 & 81.4 & 80.2 & 79 & 77.9 & 77.2 & 76 & 75.2 & 74.3 & 73.8 & 72.8 & 71.8 & 71 & 70.5 & 70.2 & 69.7\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 85.6 & 85.7 & 85.7 & 85.7 & 85.7 & 85.7 & 85.6 & 85.5 & 85.4 & 85.2 & 85 & 84.7 & 84.4 & 84.1 & 83.8 & 83.5 & 83.2 & 82.8 & 82.5 & 82.2 & 81.8 & 81.5 & 81.2 & 80.8
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 3} & $D_\alpha$   & 82.7 & 82 & 81.7 & 81.6 & 81.4 & 81.5 & 81.8 & 81.6 & 81.7 & 81.6 & 81.2 & 80.9 & 80.4 & 80.4 & 80 & 79.3 & 79 & 78.3 & 77.8 & 77.1 & 76.6 & 76.1 & 75.5 & 75.0\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.6 & 84.7 & 84.6 & 84.5 & 84.5 & 84.5 & 83.7 & 82.9 & 81.8 & 80.9 & 79.9 & 79 & 78 & 77.6 & 76.6 & 75.6 & 75.1 & 74.5 & 73.8 & 72.8 & 72.2 & 71.8 & 71.1 & 70.5\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 84.6 & 84.8 & 84.8 & 84.8 & 84.8 & 84.8 & 84.8 & 84.8 & 84.7 & 84.6 & 84.4 & 84.2 & 84 & 83.7 & 83.4 & 83.1 & 82.8 & 82.5 & 82.1 & 81.8 & 81.6 & 81.3 & 80.8 & 80.4\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 100} & $D_\alpha$   & 65.4 & 65.6 & 65.6 & 65.6 & 65.7 & 65.8 & 65.9 & 66.3 & 66.4 & 66.7 & 67.3 & 67.5 & 67.7 & 67.9 & 68.1 & 68.5 & 68.7 & 68.8 & 69 & 69.2 & 69.4 & 69.5 & 69.1 & 68.9\Bstrut\\\cline{2-26}
& $D_\beta$   & 79.6 & 79.8 & 79.9 & 79.7 & 80.1 & 80.4 & 80.7 & 80.9 & 80.7 & 80.9 & 80.8 & 80.7 & 80.7 & 80.8 & 80.4 & 80.1 & 79.9 & 79.7 & 79.3 & 78.9 & 78.4 & 77.8 & 77.4 & 77.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 79.6 & 79.6 & 79.6 & 79.6 & 79.6 & 79.6 & 79.5 & 79.4 & 79.3 & 79.1 & 78.9 & 78.7 & 78.5 & 78.2 & 78 & 77.7 & 77.4 & 77.2 & 76.9 & 76.6 & 76.3 & 76 & 75.8 & 75.6
\Tstrut\\
            \midrule
             \multirow{3}{2em}{\centering 1000} & $D_\alpha$ & 64.7 & 64.9 & 64.8 & 64.9 & 65 & 65.1 & 65.3 & 65.5 & 65.9 & 66.2 & 66.7 & 67.1 & 67.1 & 67.3 & 67.5 & 67.7 & 67.9 & 68 & 68.4 & 68.3 & 68.6 & 68.7 & 68.7 & 68.3\Bstrut\\\cline{2-26} 
            & $D_\beta$ & 79.5 & 79.8 & 79.8 & 79.7 & 80.1 & 80.3 & 80.6 & 80.8 & 80.6 & 80.9 & 80.8 & 80.7 & 80.8 & 80.8 & 80.5 & 80.2 & 79.8 & 79.7 & 79.3 & 79 & 78.6 & 77.8 & 77.5 & 77.2\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN  & 67.4 & 67.7 & 67.7 & 67.8 & 67.9 & 68 & 68.2 & 72.8 & 72.8 & 72.6 & 72.6 & 72.3 & 72.3 & 71.9 & 71.7 & 71.3 & 70.7 & 70.7 & 70.4 & 70.1 & 70.1 & 70.1 & 69.7 & 69.5\Tstrut\\
            %& MHLNB &\\
            \bottomrule
        \end{tabular}
        \end{sc}
		 }
	    \end{small}
    \end{center}
\label{tab:cifar100}
\end{table*}

==> tables/tab_odin.tex <==
\begin{table*}[!htb]
	\caption{$D_\alpha$ when perturbation as in~\eqref{eq:perturb_alpha} is applied. We have set $T$ to the values in the table and varied $\epsilon$ in $\{0,~0.0002,~0.00025,~0.0003,~0.00035,$ $~0.0004,~0.0006,~0.0008, 0.001,~0.0012,$ $0.0014,~0.0016,~0.0018,~0.002,~0.0022,$ $0.0024,~0.0026,~0.0028,~0.003,~0.0032$ $0.0034,~0.0036,~0.0038,~0.004\}$; $\epsilon^*$ denotes the $\epsilon$ with which the best AUROC is reached w.r.t. $T$.}
	\begin{center}
		\begin{small}
			\resizebox{.6\textwidth}{!}{
			\begin{sc}
				\begin{tabular}{c|c|c|c|c|c|c|c}
				    \toprule
					\textbf{DATASET} & \textbf{T} & \textbf{$\epsilon^*$} & \textbf{AUROC $\%$} & \textbf{DATASET} & \textbf{T} & \textbf{$\epsilon^*$} & \textbf{AUROC $\%$}\\ 
					\hline
					\midrule
					\multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR10\\\textnormal{Accuracy} $95\%$}}  
& \textbf{1} & \textbf{0.0003} & \textbf{95.4} 
& \multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 TinyImageNet\\\textnormal{Accuracy} $63\%$}} 
& \textbf{1} & \textbf{0.0006} & \textbf{86.8} \\ \cmidrule{2-4}\cmidrule{6-8}
& 1.1 & 0.0003 & 95.4 & & 1.1 & 0.0006 & 86.5 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.2 & 0.0003 & 95.4 & & 1.2 & 0.0006 & 86.3  \\\cmidrule{2-4}\cmidrule{6-8}
& 1.3 & 0.0003 & 95.3 & & 1.3 & 0.0008 & 85.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.4 & 0.0003 & 95.3 & & 1.4 & 0.0008 & 85.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.5 & 0.0003 & 95.3 & & 1.5 & 0.0008 & 85 \\\cmidrule{2-4}\cmidrule{6-8}
& 2 & 0.0003 & 95 & & 2 & 0.0008 & 82.7 \\\cmidrule{2-4}\cmidrule{6-8}
& 2.5 & 0.0002 & 94.6 & & 2.5 & 0 & 80.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 3 & 0.0003 & 94 & & 3 & 0 & 79.2 \\\cmidrule{2-4}\cmidrule{6-8}
& 100 & 0.0014 & 83.6 & & 100 & 0.0016 & 51.2 \\\cmidrule{2-4}\cmidrule{6-8}
& 1000 & 0.0016 & 83.1 & & 1000 & 0.0016 & 50.8\\
\midrule
\multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 CIFAR100\\\textnormal{Accuracy} $78\%$}}
& \textbf{1} & \textbf{0.00035} & \textbf{88.2} & \multirow{10}{*}{\parbox[t][][c]{3cm}{\centering
 SVHN\\\textnormal{Accuracy} $96\%$}}  
& \textbf{1} & \textbf{0.001} & \textbf{93.9} \\ 
\cmidrule{2-4}\cmidrule{6-8}
& 1.1 & 0.00035 & 88.2 & & 1.1 & 0.001 & 93.8\\\cmidrule{2-4}\cmidrule{6-8}
& 1.2 & 0.00035 & 87.9 & & 1.2 & 0.001 & 93.8 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.3 & 0.0004 & 87.8 & & 1.3 & 0.001 & 93.7  \\\cmidrule{2-4}\cmidrule{6-8}
& 1.4 & 0.0004 & 87.5 & & 1.4 & 0.001 & 93.6 \\\cmidrule{2-4}\cmidrule{6-8}
& 1.5 & 0.0004 & 87.2 & & 1.5 & 0.001 & 93.5 \\\cmidrule{2-4}\cmidrule{6-8}
& 2 & 0 & 85.6 & & 2 & 0.0012 & 92.7\\\cmidrule{2-4}\cmidrule{6-8}
& 2.5 & 0 & 84.1 & & 2.5 & 0.001 & 92  \\\cmidrule{2-4}\cmidrule{6-8}
& 3 & 0 & 82.6 & & 3 & 0.001 & 91.3 \\\cmidrule{2-4}\cmidrule{6-8}
& 100 & 0.0036 & 69.4 & & 100 & 0.0034 & 84.4 \\\cmidrule{2-4}\cmidrule{6-8}
& 1000 & 0.0036 & 68.7 & & 1000 & 0.0034 & 84\\
\bottomrule
				    \end{tabular}
			    \end{sc}
		    }
	    \end{small}
    \end{center}
\label{tab:odin}
\end{table*}

==> tables/tab_svhn.tex <==
\begin{table*}[!htb]
	\caption{Summative results: SVHN}
	\begin{center}
		\begin{small}
			\resizebox{0.9\textwidth}{!}{
			\begin{sc}
			\begin{tabular}{cl|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
            \toprule
            \multicolumn{26}{c}{\textbf{AUROC $\%$}}\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{2}{2em}{\centering T} & \multirow{2}{2em}{\centering Method} & \multicolumn{24}{c}{$\epsilon$}\\
            \cline{3-26}
            %\cmidrule[\heavyrulewidth]{3-26}
            && 0 & .0002 & .00025 & .0003 & .00035 & .0004 & .0006 & .0008 & .001 & .0012 & .0014 & .0016 & .0018 &
                .002 & .0022 & .0024 & .0026 & .0028 & .003 & .0032 & .0034 & .0036 & .0038 & .004\Tstrut\Bstrut\\
            \hline
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{4}{2em}{\centering 1} & $D_\alpha$   & 92.3 & 92.6 & 92.7 & 92.8 & 92.9 & 93 & 93.3 & 93.5 & 93.9 & 93.9 & 93.7 & 93.2 & 92.6 & 92 & 91.3 & 90.7 & 90 & 89.1 & 88.2 & 87.3 & 86.2 & 85.2 & 84.3 & 83.3\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.2 & 92.5 & 92.6 & 92.7 & 92.9 & 93 & 93.3 & 93.5 & 93.8 & 93.7 & 93.5 & 92.9 & 92.4 & 91.6 & 90.9 & 90.3 & 89.5 & 88.6 & 87.6 & 86.7 & 85.7 & 84.6 & 83.7 & 82.7\Tstrut\Bstrut\\\cline{2-26}
            & SR &  92.3 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - &-\Tstrut\Bstrut\\\cline{2-26}
            & ODIN   & 92.3 & 92.2 & 92.2 & 92.1 & 92.1 & 92 & 91.9 & 91.7 & 91.5 & 91.1 & 90.9 & 90.5 & 90.2 & 90 & 89.8 & 89.5 & 89.2 & 89 & 88.8 & 88.5 & 88.3 & 88.1 & 87.8 & 87.3\Tstrut\Bstrut\\\cline{2-26} 
            & MHLNB & 88 & 88 & 88.1 & 88.1 & 88.3 & 88.3 & 88.6 & 88.6 & 88.4 & 87.9 & 87.4 & 86.6 & 85.6 & 84.6 & 83.3 & 82.1 & 80.9 & 79.5 & 78.1 & 76.8 & 75.5 & 74.2 & 72.9 & 71.8\Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{3}{2em}{\centering 1.1} & $D_\alpha$   & 92.3 & 92.5 & 92.6 & 92.7 & 92.8 & 92.9 & 93.3 & 93.5 & 93.9 & 93.8 & 93.6 & 93.2 & 92.6 & 92 & 91.3 & 90.7 & 90.1 & 89.1 & 88.3 & 87.4 & 86.4 & 85.4 & 84.5 & 83.5\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.3 & 92.6 & 92.6 & 92.7 & 92.9 & 93 & 93.3 & 93.4 & 93.8 & 93.7 & 93.5 & 92.9 & 92.4 & 91.6 & 91 & 90.3 & 89.6 & 88.6 & 87.7 & 86.8 & 85.8 & 84.7 & 83.8 & 82.8\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 92.3 & 92.2 & 92.2 & 92.1 & 92.1 & 92 & 91.8 & 91.6 & 91.4 & 91.1 & 90.9 & 90.7 & 90.3 & 90.1 & 89.9 & 89.7 & 89.4 & 89.2 & 89 & 88.8 & 88.6 & 88.4 & 88.2 & 88.1
\Tstrut\\
            %& MHLNB & \Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.2} & $D_\alpha$   & 92.3 & 92.5 & 92.5 & 92.6 & 92.8 & 92.8 & 93.2 & 93.5 & 93.8 & 93.8 & 93.5 & 93.1 & 92.6 & 92 & 91.4 & 90.8 & 90.1 & 89.2 & 88.4 & 87.4 & 86.5 & 85.5 & 84.6 & 83.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.3 & 92.6 & 92.6 & 92.8 & 92.9 & 93 & 93.3 & 93.5 & 93.8 & 93.7 & 93.4 & 92.9 & 92.3 & 91.6 & 90.9 & 90.3 & 89.5 & 88.6 & 87.8 & 86.8 & 85.9 & 84.8 & 83.9 & 82.8\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 92.3 & 92.2 & 92.1 & 92.1 & 92 & 92 & 91.8 & 91.6 & 91.3 & 91.1 & 90.8 & 90.6 & 90.3 & 90 & 89.8 & 89.6 & 89.4 & 89.2 & 89 & 88.8 & 88.6 & 88.5 & 88.3 & 88.1\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{4}{2em}{\centering 1.3} & $D_\alpha$   & 92.2 & 92.4 & 92.4 & 92.5 & 92.7 & 92.7 & 93.1 & 93.4 & 93.7 & 93.7 & 93.4 & 93 & 92.6 & 92 & 91.4 & 90.8 & 90.1 & 89.3 & 88.5 & 87.5 & 86.7 & 85.7 & 84.8 & 84.0\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.2 & 92.5 & 92.6 & 92.7 & 92.8 & 93 & 93.2 & 93.4 & 93.7 & 93.6 & 93.4 & 92.9 & 92.3 & 91.6 & 90.9 & 90.3 & 89.5 & 88.6 & 87.8 & 86.7 & 85.9 & 84.9 & 83.9 & 83.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 92.3 & 92.1 & 92.1 & 92.1 & 92 & 92 & 91.8 & 91.5 & 91.3 & 91 & 90.8 & 90.5 & 90.2 & 90 & 89.7 & 89.5 & 89.3 & 89.1 & 88.9 & 88.7 & 88.6 & 88.4 & 88.2 & 88.1\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.4} & $D_\alpha$   & 92.1 & 92.4 & 92.4 & 92.4 & 92.6 & 92.6 & 93.1 & 93.3 & 93.6 & 93.5 & 93.3 & 93 & 92.6 & 91.9 & 91.3 & 90.7 & 90 & 89.3 & 88.5 & 87.6 & 86.7 & 85.8 & 84.9 & 84.1\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.2 & 92.5 & 92.6 & 92.7 & 92.8 & 92.9 & 93.2 & 93.4 & 93.7 & 93.6 & 93.3 & 92.8 & 92.3 & 91.6 & 90.9 & 90.3 & 89.5 & 88.7 & 87.8 & 86.8 & 85.9 & 84.9 & 84 & 83.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 92.2 & 92.1 & 92 & 92 & 92 & 91.9 & 91.7 & 91.5 & 91.2 & 91 & 90.7 & 90.4 & 90.2 & 89.9 & 89.7 & 89.4 & 89.2 & 89 & 88.8 & 88.6 & 88.4 & 88.3 & 88.1 & 88.0\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 1.5} & $D_\alpha$   & 92.1 & 92.3 & 92.3 & 92.4 & 92.5 & 92.5 & 92.9 & 93.1 & 93.5 & 93.4 & 93.2 & 92.9 & 92.5 & 91.9 & 91.3 & 90.7 & 90 & 89.3 & 88.5 & 87.6 & 86.8 & 85.9 & 85.1 & 84.3\Bstrut\\\cline{2-26}
& $D_\beta$   & 92.2 & 92.4 & 92.5 & 92.6 & 92.8 & 92.9 & 93.2 & 93.3 & 93.7 & 93.6 & 93.3 & 92.7 & 92.2 & 91.6 & 90.8 & 90.2 & 89.4 & 88.6 & 87.7 & 86.8 & 85.9 & 84.9 & 84 & 83.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 92.2 & 92 & 92 & 92 & 91.9 & 91.9 & 91.7 & 91.4 & 91.2 & 90.9 & 90.6 & 90.3 & 90.1 & 89.8 & 89.6 & 89.3 & 89.1 & 88.9 & 88.7 & 88.5 & 88.3 & 88.1 & 88 & 87.8
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2} & $D_\alpha$   & 91.6 & 91.8 & 91.9 & 91.9 & 92 & 92.1 & 92.4 & 92.5 & 92.7 & 92.7 & 92.6 & 92.2 & 91.8 & 91.4 & 90.9 & 90.4 & 89.7 & 89.2 & 88.5 & 87.7 & 86.9 & 86.1 & 85.4 & 84.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 91.9 & 92.2 & 92.2 & 92.4 & 92.5 & 92.6 & 92.9 & 93.1 & 93.3 & 93.1 & 92.9 & 92.4 & 91.9 & 91.2 & 90.5 & 89.8 & 89.1 & 88.4 & 87.6 & 86.6 & 85.7 & 84.8 & 84.1 & 83.3\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 91.9 & 91.8 & 91.7 & 91.7 & 91.6 & 91.6 & 91.3 & 91.1 & 90.8 & 90.5 & 90.2 & 89.9 & 89.7 & 89.4 & 89.1 & 88.8 & 88.6 & 88.4 & 88.1 & 87.9 & 87.7 & 87.6 & 87.4 & 87.2
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2.5} & $D_\alpha$   & 91.1 & 91.2 & 91.2 & 91.4 & 91.4 & 91.5 & 91.7 & 91.8 & 92 & 92 & 91.8 & 91.5 & 91.2 & 90.7 & 90.4 & 89.9 & 89.4 & 88.8 & 88.2 & 87.5 & 86.8 & 86.1 & 85.4 & 84.8\Bstrut\\\cline{2-26}
& $D_\beta$   & 91.7 & 91.9 & 92 & 92.1 & 92.2 & 92.3 & 92.6 & 92.8 & 92.9 & 92.8 & 92.5 & 92 & 91.4 & 90.8 & 90.2 & 89.5 & 88.8 & 88.1 & 87.4 & 86.5 & 85.6 & 84.7 & 84.1 & 83.3\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 91.7 & 91.5 & 91.4 & 91.4 & 91.3 & 91.3 & 91 & 90.8 & 90.5 & 90.2 & 89.9 & 89.6 & 89.3 & 89 & 88.7 & 88.4 & 88.1 & 87.9 & 87.7 & 87.4 & 87.2 & 87 & 86.9 & 86.7
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 3} & $D_\alpha$   & 90.6 & 90.6 & 90.7 & 90.8 & 90.8 & 90.9 & 91 & 91.1 & 91.3 & 91.3 & 91.1 & 90.8 & 90.6 & 90.2 & 89.8 & 89.5 & 89 & 88.6 & 88.1 & 87.4 & 86.8 & 86.1 & 85.5 & 84.8\Bstrut\\\cline{2-26}
& $D_\beta$   & 91.4 & 91.7 & 91.7 & 91.8 & 92 & 92.1 & 92.4 & 92.5 & 92.7 & 92.5 & 92.2 & 91.7 & 91.1 & 90.6 & 89.9 & 89.3 & 88.6 & 87.9 & 87.2 & 86.4 & 85.5 & 84.7 & 84.2 & 83.4\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 91.4 & 91.2 & 91.2 & 91.1 & 91.1 & 91 & 90.7 & 90.5 & 90.2 & 89.9 & 89.6 & 89.2 & 88.9 & 88.6 & 88.3 & 88 & 87.8 & 87.5 & 87.3 & 87 & 86.8 & 86.6 & 86.4 & 86.2\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 100} & $D_\alpha$   & 79.2 & 79.6 & 79.7 & 79.8 & 79.7 & 79.8 & 80.1 & 80.5 & 80.6 & 81.1 & 81.6 & 82.1 & 82.4 & 82.9 & 83 & 83.4 & 83.8 & 84 & 84.2 & 84.3 & 84.5 & 84.4 & 84.4 & 84.4\Bstrut\\\cline{2-26}
& $D_\beta$   & 89.5 & 89.8 & 89.8 & 89.9 & 90.1 & 90.2 & 90.6 & 90.6 & 90.7 & 90.5 & 90.5 & 90.1 & 89.7 & 89.3 & 88.8 & 88.4 & 88 & 87.5 & 87.1 & 86.6 & 85.9 & 85.4 & 84.8 & 84.2\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 89.5 & 89.2 & 89.2 & 89.1 & 89 & 88.9 & 88.6 & 88.3 & 88 & 87.6 & 87.2 & 86.9 & 86.5 & 86.2 & 85.8 & 85.5 & 85.1 & 84.8 & 84.5 & 84.3 & 84 & 83.7 & 83.5 & 83.3
\Tstrut\\
            \midrule
             \multirow{3}{2em}{\centering 1000} & $D_\alpha$ & 64.7 & 64.9 & 64.8 & 64.9 & 65 & 65.1 & 65.3 & 65.5 & 65.9 & 66.2 & 66.7 & 67.1 & 67.1 & 67.3 & 67.5 & 67.7 & 67.9 & 68 & 68.4 & 68.3 & 68.6 & 68.7 & 68.7 & 68.3\Bstrut\\\cline{2-26} 
            & $D_\beta$ & 89.4 & 89.7 & 89.8 & 89.9 & 90.1 & 90.2 & 90.6 & 90.6 & 90.6 & 90.5 & 90.4 & 90.1 & 89.6 & 89.3 & 88.8 & 88.4 & 88 & 87.5 & 87.1 & 86.6 & 86 & 85.4 & 84.9 & 84.3\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN & 88.9 & 88.7 & 88.6 & 88.5 & 88.5 & 88.4 & 88.1 & 87.7 & 87.4 & 87.2 & 86.7 & 86.2 & 85.9 & 85.6 & 85.2 & 84.8 & 84.4 & 84.2 & 84.1 & 83.8 & 83.6 & 83.3 & 83 & 82.8\Tstrut\\
            %& MHLNB &\\
            \bottomrule
        \end{tabular}
        \end{sc}
		 }
	    \end{small}
    \end{center}
\label{tab:svhn}
\end{table*}

==> tables/tab_tinyimagenet.tex <==
\begin{table*}[!htb]
	\caption{Summative results: TinyImageNet}
	\begin{center}
		\begin{small}
			\resizebox{0.9\textwidth}{!}{
			\begin{sc}
			\begin{tabular}{cl|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
            \toprule
            \multicolumn{26}{c}{\textbf{AUROC $\%$}}\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{2}{2em}{\centering T} & \multirow{2}{2em}{\centering Method} & \multicolumn{24}{c}{$\epsilon$}\\
            \cline{3-26}
            %\cmidrule[\heavyrulewidth]{3-26}
            && 0 & .0002 & .00025 & .0003 & .00035 & .0004 & .0006 & .0008 & .001 & .0012 & .0014 & .0016 & .0018 &
                .002 & .0022 & .0024 & .0026 & .0028 & .003 & .0032 & .0034 & .0036 & .0038 & .004\Tstrut\Bstrut\\
            \hline
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{4}{2em}{\centering 1} & $D_\alpha$   & 84.9 & 85.5 & 85.7 & 85.8 & 86.1 & 86.2 & 86.8 & 86.4 & 85.7 & 84.6 & 83.4 & 82 & 80.8 & 79.8 & 78.5 & 77.4 & 76.2 & 74.8 & 73.8 & 72.9 & 71.8 & 70.8 & 70 & 69.2\Bstrut\\\cline{2-26}
            & $D_\beta$   & 84.9 & 85.6 & 85.6 & 85.7 & 86 & 86 & 86 & 84.8 & 83.9 & 82.2 & 80.6 & 79.2 & 77.8 & 76.5 & 75.2 & 74 & 72.7 & 71.6 & 70.8 & 70 & 68.9 & 67.8 & 67.4 & 66.6\Tstrut\Bstrut\\\cline{2-26}
            & SR & 84.9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - &-\Tstrut\Bstrut\\\cline{2-26}
            & ODIN  & 84.9 & 84.9 & 84.9 & 84.9 & 84.9 & 84.8 & 84.7 & 84.6 & 84.4 & 84.3 & 84.2 & 84.1 & 84 & 83.8 & 83.7 & 83.6 & 83.5 & 83.5 & 83.4 & 83.3 & 83.2 & 83.1 & 83 & 82.9\Tstrut\Bstrut\\\cline{2-26}
            & MHLNB & 58.9 & 58.8 & 58.9 & 58.8 & 58.7 & 58.7 & 58.2 & 57.4 & 56.3 & 55.6 & 54.9 & 54.2 & 53.7 & 53 & 52.4 & 51.8 & 51.3 & 50.5 & 49.9 & 49.4 & 49 & 48.7 & 48.2 & 47.8\Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
            \multirow{3}{2em}{\centering 1.1} & $D_\alpha$   & 84.9 & 85.4 & 85.5 & 85.7 & 85.8 & 86 & 86.6 & 86.3 & 85.8 & 84.7 & 83.7 & 82.4 & 81.2 & 80.2 & 79.1 & 78.1 & 76.8 & 75.6 & 74.5 & 73.4 & 72.4 & 71.4 & 70.5 & 69.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.9 & 85.6 & 85.6 & 85.7 & 86 & 86.1 & 85.9 & 84.9 & 83.9 & 82.4 & 80.8 & 79.5 & 78.1 & 76.9 & 75.7 & 74.7 & 73.4 & 72.1 & 71.2 & 70 & 69.3 & 68.4 & 67.7 & 66.9\Tstrut\Bstrut\\\cline{2-26}
& ODIN  & 84.9 & 84.9 & 84.9 & 84.9 & 84.9 & 84.9 & 84.7 & 84.6 & 84.5 & 84.3 & 84.2 & 84.1 & 84 & 83.9 & 83.8 & 83.7 & 83.6 & 83.5 & 83.4 & 83.3 & 83.3 & 83.2 & 83.1 & 83.0\Tstrut\\
            %& MHLNB & \Tstrut\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.2} & $D_\alpha$   & 84.7 & 85.1 & 85.2 & 85.4 & 85.4 & 85.7 & 86.3 & 86.2 & 85.6 & 84.7 & 83.8 & 82.6 & 81.4 & 80.4 & 79.5 & 78.4 & 77.2 & 76.1 & 74.9 & 74 & 72.9 & 72 & 71 & 70.2\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.9 & 85.5 & 85.5 & 85.6 & 85.8 & 85.9 & 85.8 & 85 & 83.9 & 82.6 & 81.1 & 79.7 & 78.4 & 77.1 & 76.3 & 75.1 & 73.7 & 72.5 & 71.4 & 70.6 & 69.8 & 68.8 & 68 & 67.3\Tstrut\Bstrut\\\cline{2-26}
& ODIN  & 84.9 & 84.9 & 84.9 & 84.9 & 84.9 & 84.8 & 84.7 & 84.6 & 84.5 & 84.4 & 84.2 & 84.1 & 84 & 83.9 & 83.8 & 83.7 & 83.6 & 83.5 & 83.5 & 83.4 & 83.3 & 83.2 & 83.1 & 83.1
\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{4}{2em}{\centering 1.3}& $D_\alpha$   & 84.5 & 84.9 & 85 & 85.1 & 85.2 & 85.3 & 85.8 & 85.9 & 85.3 & 84.6 & 83.4 & 82.5 & 81.3 & 80.5 & 79.9 & 78.8 & 77.7 & 76.5 & 75.5 & 74.3 & 73.3 & 72.5 & 71.5 & 70.6\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.8 & 85.4 & 85.4 & 85.5 & 85.7 & 85.8 & 85.7 & 84.8 & 83.8 & 82.6 & 81.4 & 80 & 78.7 & 77.3 & 76.5 & 75.4 & 74.1 & 72.9 & 71.9 & 70.9 & 70 & 69.2 & 68.4 & 67.8\Tstrut\Bstrut\\\cline{2-26}
& ODIN  & 84.9 & 84.9 & 84.8 & 84.8 & 84.8 & 84.8 & 84.7 & 84.6 & 84.5 & 84.3 & 84.2 & 84.1 & 84 & 83.9 & 83.8 & 83.7 & 83.6 & 83.5 & 83.5 & 83.4 & 83.3 & 83.2 & 83.2 & 83.1
\Tstrut\\
            %& MHLNB &\\
            \cmidrule[\heavyrulewidth]{1-26}
             \multirow{3}{2em}{\centering 1.4} & $D_\alpha$   & 84.3 & 84.5 & 84.5 & 84.8 & 84.8 & 84.9 & 85.3 & 85.5 & 84.8 & 84.1 & 83.1 & 82.3 & 81.3 & 80.6 & 79.8 & 78.8 & 77.9 & 76.6 & 75.8 & 74.7 & 73.7 & 72.7 & 72.1 & 71.1\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.7 & 85.3 & 85.3 & 85.3 & 85.5 & 85.7 & 85.7 & 84.8 & 83.8 & 82.7 & 81.4 & 80.2 & 78.7 & 77.6 & 77 & 75.6 & 74.4 & 73.1 & 72.1 & 71.1 & 70.2 & 69.4 & 68.8 & 68.1\Tstrut\Bstrut\\\cline{2-26}
& ODIN  & 84.8 & 84.8 & 84.8 & 84.7 & 84.7 & 84.7 & 84.6 & 84.5 & 84.4 & 84.3 & 84.2 & 84.1 & 84 & 83.9 & 83.8 & 83.7 & 83.6 & 83.5 & 83.4 & 83.4 & 83.3 & 83.2 & 83.2 & 83.1
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 1.5} & $D_\alpha$   & 84.1 & 84.1 & 84.3 & 84.4 & 84.3 & 84.4 & 84.8 & 85.1 & 84.4 & 83.7 & 82.9 & 82 & 81.4 & 80.5 & 79.8 & 78.8 & 78.1 & 76.9 & 75.9 & 74.9 & 73.9 & 73.1 & 72.3 & 71.4\Bstrut\\\cline{2-26}
& $D_\beta$   & 84.6 & 85.1 & 85.1 & 85.2 & 85.3 & 85.5 & 85.4 & 84.6 & 83.7 & 82.6 & 81.6 & 80.2 & 78.8 & 77.8 & 77.1 & 75.9 & 74.7 & 73.5 & 72.4 & 71.4 & 70.3 & 69.6 & 69.1 & 68.2\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 84.6 & 84.6 & 84.6 & 84.6 & 84.6 & 84.6 & 84.5 & 84.4 & 84.3 & 84.2 & 84.1 & 84 & 83.9 & 83.8 & 83.7 & 83.7 & 83.6 & 83.5 & 83.4 & 83.3 & 83.2 & 83.2 & 83.1 & 83.0
\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2} & $D_\alpha$   & 82.5 & 82.3 & 82.3 & 82.4 & 82.3 & 82.3 & 82.5 & 82.8 & 82.5 & 82 & 81.6 & 80.9 & 80.2 & 79.4 & 79.3 & 78.4 & 77.6 & 77 & 75.9 & 75.1 & 74.2 & 73.7 & 72.8 & 72.2\Bstrut\\\cline{2-26}
& $D_\beta$   & 83.8 & 84.1 & 84.3 & 84.3 & 84.4 & 84.4 & 84.6 & 83.9 & 82.9 & 82.2 & 81.2 & 80 & 79 & 78 & 77.2 & 76.1 & 75.1 & 74.3 & 73.2 & 72.1 & 71.3 & 70.5 & 69.8 & 69.2\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 83.8 & 83.9 & 83.9 & 83.9 & 83.9 & 83.9 & 83.8 & 83.8 & 83.7 & 83.7 & 83.6 & 83.5 & 83.5 & 83.4 & 83.3 & 83.2 & 83.2 & 83.1 & 83 & 83 & 82.9 & 82.8 & 82.8 & 82.7\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 2.5} & $D_\alpha$   & 80.8 & 80.5 & 80.5 & 80.4 & 80.4 & 80.3 & 80 & 80.2 & 80.3 & 80.2 & 79.5 & 79.2 & 78.5 & 78.1 & 77.8 & 77.1 & 76.6 & 75.9 & 75.2 & 74.5 & 73.4 & 72.3 & 71.6 & 70.7\Bstrut\\\cline{2-26}
& $D_\beta$   & 83 & 83.2 & 83.4 & 83.5 & 83.7 & 83.5 & 83.7 & 83.3 & 82.5 & 81.8 & 80.9 & 80 & 78.9 & 78.1 & 77.3 & 76.2 & 75.3 & 74.6 & 73.6 & 72.7 & 71.9 & 71.1 & 70.3 & 69.6\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 83 & 83.1 & 83.1 & 83.1 & 83.1 & 83.1 & 83.1 & 83.1 & 83 & 83 & 82.9 & 82.9 & 82.8 & 82.8 & 82.7 & 82.7 & 82.6 & 82.6 & 82.5 & 82.4 & 82.4 & 82.3 & 82.3 & 82.2\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 3} & $D_\alpha$   & 79.2 & 78.9 & 78.8 & 78.7 & 78.7 & 78.5 & 78.4 & 78.1 & 78.2 & 78.2 & 77.8 & 77.4 & 76.7 & 76.2 & 75.8 & 75.5 & 74.9 & 74.2 & 73.4 & 72.9 & 71.8 & 71.2 & 70.4 & 69.5\Bstrut\\\cline{2-26}
& $D_\beta$   & 82.4 & 82.6 & 82.8 & 82.8 & 83.1 & 83 & 83.1 & 82.9 & 82 & 81.6 & 80.7 & 80 & 78.9 & 78.3 & 77.5 & 76.5 & 75.8 & 74.9 & 74.1 & 73.1 & 72.3 & 71.5 & 70.7 & 69.9\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 82.4 & 82.5 & 82.5 & 82.5 & 82.5 & 82.5 & 82.5 & 82.5 & 82.5 & 82.4 & 82.4 & 82.3 & 82.3 & 82.2 & 82.2 & 82.1 & 82.1 & 82 & 82 & 81.9 & 81.9 & 81.8 & 81.8 & 81.7\Tstrut\\
            %& MHLNB &\\
             \midrule
             \multirow{3}{2em}{\centering 100} & $D_\alpha$   & 50.4 & 50.5 & 50.5 & 50.5 & 50.6 & 50.7 & 50.9 & 51.1 & 50.9 & 50.9 & 51 & 51.1 & 51 & 50.9 & 51 & 51 & 51 & 50.7 & 50.8 & 50.6 & 50.4 & 50.3 & 50.1 & 49.8\Bstrut\\\cline{2-26}
& $D_\beta$   & 80.1 & 80.3 & 80.3 & 80.6 & 80.7 & 80.9 & 81 & 81 & 80.4 & 80.1 & 79.7 & 79.2 & 78.5 & 77.6 & 77.3 & 76.4 & 75.7 & 74.9 & 74.1 & 73.8 & 72.7 & 71.6 & 70.8 & 70.0\Tstrut\Bstrut\\\cline{2-26}
& ODIN   & 78.9 & 80.1 & 80.1 & 80.1 & 80.1 & 80.1 & 80 & 80 & 79.9 & 79.8 & 79.8 & 79.7 & 79.7 & 79.6 & 79.5 & 79.5 & 79.4 & 79.4 & 79.3 & 79.3 & 79.2 & 79.2 & 79.1 & 79.1\Tstrut\\
            \midrule
             \multirow{3}{2em}{\centering 1000} & $D_\alpha$ & 64.7 & 64.9 & 64.8 & 64.9 & 65 & 65.1 & 65.3 & 65.5 & 65.9 & 66.2 & 66.7 & 67.1 & 67.1 & 67.3 & 67.5 & 67.7 & 67.9 & 68 & 68.4 & 68.3 & 68.6 & 68.7 & 68.7 & 68.3\Bstrut\\\cline{2-26} 
            & $D_\beta$  & 80 & 80.2 & 80.2 & 80.6 & 80.7 & 80.9 & 81 & 80.9 & 80.4 & 80.1 & 79.6 & 79.2 & 78.5 & 77.6 & 77.3 & 76.4 & 75.7 & 74.9 & 74.1 & 73.7 & 72.7 & 71.6 & 70.8 & 70.1\Tstrut\Bstrut\\ \cline{2-26}
            & ODIN & 80 & 80 & 80 & 80 & 80 & 80 & 80 & 79.9 & 79.8 & 79.8 & 79.7 & 79.6 & 79.6 & 79.5 & 79.5 & 79.4 & 79.4 & 79.3 & 79.2 & 79.2 & 79.1 & 79.1 & 79.1 & 79.1\Tstrut\\
            %& MHLNB &\\
            \bottomrule
        \end{tabular}
        \end{sc}
		 }
	    \end{small}
    \end{center}
\label{tab:tiny}
\end{table*}
